Asymptotic properties of one-layer artificial neural networks with sparse connectivity

A law of large numbers for the empirical distribution of parameters of a one-layer artificial neural networks with sparse connectivity is derived for a simultaneously increasing number of both, neurons and training iterations of the stochastic gradient descent.

==> compact.tex <==
\subsection{Relative compactness}
In this section, we show relative compactness of the sequence $\{\LL(\mu^N)\}_{N \ge 1}$ in the space $\MM(D_E([0, T]))$.

%
%REL COMP
%
\bepr[Relative compactness]
\label{rel_comp_prop}
The sequence  $\{\LL(\mu^N)\}_{N \ge 1}$ is relatively compact
\enpr

To prove Proposition \ref{rel_comp_prop}, we need compact containment and regularity.

%
%COMP CONT
%
\bel[Compact containment]
\label{marge_tight_lem}
Let $\e > 0$. There exists compact $K$ such that
$$\sup_{N, t\le T}\E[\mu_t^N \not \in K] < \e$$
\enl

%
%REG
%
For the regularity, we set 
$$q(z_1, z_2) := |z_1 - z_2| \wedge 1$$
\bel[Regularity]
\label{reg_lem}
We have that for all $ u,v\le \de$ 
$$\E\big[q(\lf{\mu_{t + u}^N}, \lf{\mu_t^N} )q(\lf{\mu_{t + u}^N}, \lf{\mu_{t - v}^N} )\,|\,\FF_t\big] \le C\de^p + \frac CN.$$
\enl

%
%REL COMP PRF
%
With these Lemmas, we prove Proposition \ref{rel_comp_prop}.
\bep[Proof of Proposition \ref{rel_comp_prop}]
At this point, we may need to be a bit careful for the following technical reason. In \cite{kurtz} $\FF_t$ refers to the filtration generated by the process. However, if we can show that all estimates also hold uniformly conditioned on the initial distribution, then we should be good.

Invoking \cite[Theorem 8.6]{kurtz}, the assertion follows from Lemmas \ref{bound_lem} and \ref{reg_lem}.
\enp

%
%MARGE PRF
%
Now, we prove Lemma \ref{marge_tight_lem}.
\bep[Proof of Lemma \ref{marge_tight_lem}]
TBA.
\enp

%
%REG PRF
%
\bep[Proof of Lemma \ref{reg_lem}]
By Taylor expansion, we obtain that
$$|\lf{\mu_t^N} - \lf{\mu_s^N}| \le \frac1N\sum_i||\nabla_w f(\bar c_{Nt}^i, \bar w_{Nt}^i)||\cdot||w_{Nt}^i - w_{Nt}^i||.$$

We bound the expectation of the $||w_{Nt}^i - w_{Ns}^i||$ as follows. 
\begin{align*}
||w_{Nt}^i - w_{Ns}^i||\le \frac1N\sum_{Ns \le k \le Nt} ||\a (Y_k - g_{\theta_k}(X_k))c_k^i\s'(w_k^iX_k)x_k(\Xi^i)||
\end{align*}
Since we assumed that $\pi$ is compactly supported, everything remains bounded here.
\enp
